A Graph Attention Learning Approach to Antenna Tilt Optimization

6G will move mobile networks towards increasing levels of complexity. To deal with this complexity, optimization of network parameters is key to ensure high performance and timely adaptivity to dynamic network environments. The optimization of the antenna tilt provides a practical and cost-efficient method to improve coverage and capacity in the network. Previous methods based on Reinforcement Learning (RL) have shown great promise for tilt optimization by learning adaptive policies outperforming traditional tilt optimization methods. However, most existing RL methods are based on single-cell features representation, which fails to fully characterize the agent state, resulting in suboptimal performance. Also, most of such methods lack scalability, due to state-action explosion, and generalization ability. In this paper, we propose a Graph Attention Q-learning (GAQ) algorithm for tilt optimization. GAQ relies on a graph attention mechanism to select relevant neighbors information, improve the agent state representation, and update the tilt control policy based on a history of observations using a Deep Q-Network (DQN). We show that GAQ efficiently captures important network information and outperforms standard DQN with local information by a large margin. In addition, we demonstrate its ability to generalize to network deployments of different sizes and densities.

==> deleted_text.tex <==
%\subsection{Evaluation metrics}
%The reward is a function of the normalized variation between KPIs in the network at the end of the episode $KPI_{fin}$ comparing with its value at the beginning $KPI_{init}$. In our formulation, we specify such KPI to be the combination of 2 factors, Traffic share of good traffic $T_\%$, and RRC congestion rate $C_{RRC}$. Traffic share denotes the ratio of good traffic, for both the optimising antenna and its neighbors, comparing with all transmitted data traffic amount. The threshold of good $Tg_i$ /bad traffic $Tb_i$ is align with the simulation environment configuration in \ref{subsec:sim}:
%\begin{equation}
%\label{eql:KPI Reward}
%  r = \frac{KPI_{fin} -KPI_{init}}{{KPI}}
%\end{equation}
%\begin{equation}
%\label{eql:TS}
%  T_\%_i = \frac{Tg_i}{2(Tg_i + Tb_i)} + \frac{\sum_{j \in N(c_i)}Tg_j}{2\sum_{j \in N(c_i)}(Tg_j+Tb_j)}
%\end{equation}
%\begin{equation}
%\label{eql:TS}
%  KPI_i = T_\%_i - \frac{C_{RRC}_i}{2} - \frac{\sum_{j \in N(c_i)}C_{RRC}_j}{2}
%\end{equation}
%We have also used the standalone $T_g$, $T_b$ and $C_{RRC}$ as optional evaluation metric of the baselines.

%\item We apply offset $b_{ii} = \log ((N-1) (\frac{1}{1-b_0} -1))$ (where $b_0$ is initial coefficient to be configured as hyper-parameter) on the diagonal elements of the attention $\Lambda = \text{diag}(\alpha^{m}_{i,j})$ to strengthen the self attention (For neighboring attention, $b_{ij} = 0$). This is due to in RET optimization, the information of neighboring nodes is less important than the target node information.

%For a vector $a \in \mathbb{R}^d$, we denote the $d\times d$ diagonal matrix defined by $a$ as $\mathrm{diag}(a)$. 

%We thus formulate the problem as Decentralized Partially Observable Markov Process. In each time setup of the training, we store a tuple $(h_{t,i}, a_{t,i}, h_{t+1,i},r_{t,i})$, and the objective is to maximize the sum of all agents expected returns. 

%play a major role in improving network performance but also leads to challenges related to complex network topologies

%We have included a variety of features as input to our model. In defining the input features, we need to configure 3 hyper parameters: The Reference Signal Receiving Power (RSRP) thresh-hold defining a good/bad traffic throughput, threshold of serving-signal-to-interferer ratio (SIR) to consider an interferer as overlapping site, and a threshold of serving-SIR to be considered an interferer to be the strongest one as within interference margin.\\

% We show that GAQ has outperforms vanilla DQN, obtaining $x\%$ performance improvement. 
%To improve the KPIs aims to improve antennas' cooperation effect since KPIs measure the quality of cooperation between the antenna to be optimized and its neighbor antennas.


% GNN is an ANN acting on graph-structural input. It was first introduced by \cite{gnn_model} and many variants have been developed \cite{defferrard_convolutional_2017}. Its basic version consists of many nodes with special properties in an input graph that have initial states. The nodes connect due to potential relationships, and the links that connect them represent the relationship between nodes.
% GNN can be used to operate over graphs to achieve relational reasoning and state aggregation. That is, GNN can help facilitate illustrating the relationship among nodes which describe specific entities in the graph and representing the pattern of relations between nodes. GNN has shown  unprecedented generalization performance when applied to network modeling and network optimization.  
% GNN act on graphs to obtain a graph (or node/link) embedding. Analogous to the traditional Convolutional Neural Networks (CNNs), convolution operation on an image, the embedding of the antenna network that this paper seeks is also based on nodes' spatial relations. Images can be seen as a unique form of a graph where each pixel represents a node. Moreover, each pixel is connected to other pixels adjacent to it in an orderly manner. Image convolution slides a fixed-size convolution kernel over the image and extracts the weighted average of each central node's pixel values and its neighboring nodes on multiple channels. Similarly, space-based graph convolution convolves the representation of the concerned node and its neighbors to derive the updated representation of the concerned node. Thus, the spatial graph convolution operation can be competent for the critical task of spreading node information along edges.

% Comment from Fillipo: This section should be about theory of GNNs that is also used in our algorithm. What you write here @Yifei, is more about motivation of using GNN that should be moved elsewhere.Can you please explain about the high level function of GNNs?

% GNNs have been successful due to it constrains the input neurons the neighboring nodes.

%In the earliest years, GNN had been used to learn the target node's representation, \cite{gnn_model}, by propagating and receiving neighboring information iteratively until convergence. Such method is considered to be expensive and time-costly. With new approaches \cite{kipf2016semi}\cite{hamilton2018inductive}, developed in recent decade that being more efficient.\\
%Most recent application contributes to have GNN handles homogeneous graph. Besides its wide application in social network, traffic management and recommendation system, telecommunication network, benefited from its highly regularized structure and neighborhood homogeneity, has become a new field of GNN application. 

\begin{comment}

%\medskip \noindent \textbf{Notation.}  For any $M\in\mathbb{N}$, we define $[M] = \{1,\dots,M\}$. %For any two vectors $x,y \in\mathbb{R}^{d}$, we denote by $x||y \in\mathbb{R}^{2d}$ the concatenation operation, and for a set of vectors $(x_m)_{m\in[M]}$, we define $||_{m\in [M]} x_m = x_1||x_2||\dots ||x_M$. 

\subsection{Graph Neural Networks}
Different from conventional ANNs, GNNs broaden the input space into the geometric space, mostly from a graph representation of complex systems or networks. 
When representing complex systems, one can improve the expressiveness of the graph representation with topological patterns, nodes, edge attributes, and sub-graph features. Besides selecting the GNN architecture which captures the topological feature, one also needs to consider an \textit{embedding function} and a \textit{readout function}, that can effectively encode other features in the receptive field of GNN, and inference the embedding toward the given ground truth, respectively. Besides \textit{embedding function} and \textit{readout function}.
The GNN function can be concisely described by the following equation \cite{grl}:
\begin{equation}
\label{equ:gnn}
    h^{(k+1)}_u = \textsc{update}^{(k)}\left(h^{(k)}_u, \textsc{aggregate}^{(k)}_{v \in \mathcal{N}(u)} h^{(k)}_v\right),
\end{equation}
where $h^{(k)}_v$ denote node $v$'s embedding in $k$-th GNN layer, $\mathcal{N}(v)$ denote the adjacent node of node $v$, $\textsc{aggregate}$ denotes an aggregation function, that combines the neighbor's nodes embedding with the one of the target node $u$. $\textsc{update}$ updates the $u$-th feature embedding to its next layer embedding $h^{(k+1)}_u$.

Incorporating domain knowledge is a common practice for representing the graph. According to the nature of the formulated graph representation, GNN architecture, embedding \& readout function and reward settings are required to adjust accordingly in most applications, e.g. medicine design \cite{hu2019strategies} \& physical process simulation \cite{sanchez2020learning}. According to \citet{balcilar2020analyzing}, the graph signal posed by feature formulation dictates the generalization ability of produced embedding from GNN model, for a few modern GNN architectures \cite{kipf2016semi, hamilton2018inductive, velickovic2018gat}.

Specifically, for the domain of RET optimization, one nature is there exists significant correlation between geographically proximate sites. Such correlation can impact its both ends service quality positively if proper configured. In case of inappropriate parameters, this relation can also harm both connected parties' service quality. Some configuration parameter can strength such relation, while it fades as the inter-site distance increases, regardless of positive or negative impact it poses towards both sites. There exist a few state-of-the-art contributions \cite{schlichtkrull2018modeling,wang2019heterogeneous} tackling such heterogeneous relation, while associating the relation's heterogeneity with its connecting agents' action in RL formulation is still to be studied. This problem can be considered as a modified \textit{Set Covering Problem} and is proven to be \textit{NP-Complete} \cite{karp1972reducibility}.
%Spatial graph convolution convolves the embedding of the target node and its neighbors to update each node embedding.
%The spatial graph convolution operation can be effective for the critical task of spreading node information along edges.\\
%However, classical GCN approaches may suffer limitations that are circle in producing expressive embedding for antennas in mobile network. The information of same node pass to different neighbors can be important in different part, as well as the conventional GCN is limited in specifying different weights to different nodes in a neighborhood. Unlike previous methods, GAQ  strengthen relevant feature for each target node and can handle inductive settings for the RET optimization problem.\\
\end{comment}

%by producing the attention coefficients. This is done by using a single-layer feed-forward ANN with Leaky-ReLU activation. Finally, a softmax layer is applied to the attention coefficients to normalize them. 


%$e_{i,j} = \mathrm{LeakyReLU}(Wh_i,Wh_j)$, where $a:\mathbb{R}^{d'}\times \mathbb{R}^{d'} \to \mathbb{R}$ is a non-linear transformation. A common choice is to use a single-layer feed-forward with Leaky-ReLu activation.
%\begin{equation}
%\label{eq:attention}
%\alpha_{i j}=\operatorname{softmax}_{j}\left(e_{i j}\right)=\frac{\exp \left(e_{i j}\right)}{\sum_{k \in \mathcal{N}_{i}} \exp \left(e_{i k}\right)}.
%\end{equation}

 % Inspired by \cite{jiang2020graph}, t
%introduces neighboring attention through a masked graph attention setting. For a node  and for time $t\geq 1$, let $h_{t,i}$ be the feature vector. 
%In tilt optimization, a node is a network cell, controlled by an antenna, and $s_{t,i}$ includes a set of KPIs representing the state of the target node $i$. 
 %input feature of each node $i$: $h_{t,i} = [\theta_{t,i}, \textsc{Cov}_{t,i}, \textsc{Cap}_{t,i}, \textsc{Qual}_{t,i}]$, dataset $\mathcal{D_{\pi}}$
 % Change s_{t} with $h_{t}$
 % Have weights with w. 
 
 
 %We conduct hyper-parameter search to find the best performing model. The Hyper-parameters tuned are the Learning rate $\eta$ and the batch size $T_{\text{batch}}$. The search is executed by sampling $N_{\text{sample}} = 115$ from a log-uniform distributed for $\eta$ and a discrete uniformly for $T_{\text{batch}}$. The other parameters are kept fixed and are reported in \cref{table:otherhp}.


% \begin{table}{H}
%   \caption{Hyper parameter search configuration}
%   \label{table:hpsearch}
%   \centering 
%   \begin{threeparttable}
%     \begin{tabular}{ccc}
%     Parameter search configuration & Symbol & Value\\
%      \midrule\midrule
%     Learning Rate  & $\{{\eta}\}$&  $\mathcal{U}(\log(10^{-4}), \log(10^{-2}))$ \\
%     \midrule
%     Batch size  & $\{{N_B}\}$  &  $\mathcal{U}(10,200)$ \\
%     \midrule
%     Sample amount & ${S}$ & 115 \\
%     \midrule\midrule
%     \end{tabular}
% \end{threeparttable}
% \end{table}

  %\item In step 1, for each attention head $m\in[M]$, we introduce a feature dimension increment kernel $W^m \in \mathbb{R}^{d'\times d}$, with $d' \ge d$.
    %\item In step 2, Through $W^m$, we can produce augmented feature vectors $h^m_{t,i} =  W^m h_{t,i} \in \mathbb{R}^{d'}$.
    %\item In step 3, we compute the pair-wise attention coefficients $\alpha^{m}_{i,j} \in [0,1]$. We introduce the learnable parameter $w_a \in \mathbb{R}^{2d'}$ as in \cite{velickovic2018gat} to parametrize the pair-wise attentions. The attention coefficients represents the degree of pair-wise dependence indicator between neighboring node's feature.
    % Yifei attach a graph later to indicate this relation by illustrating the attention weight
    
    %For example, \citet{Guo13} employed a Boltzmann exploration approach in heterogeneous networks to maximize  throughput fairness, while \citet{Razavi10} proposed a fuzzy-RL method which combines  fuzzy logic to model the intrinsic uncertainty of the states in mobile cellular networks and then apply DQN to learn a good antenna tilt policy. 
    
    
%According to the method of graph structure being formulated, one can consider there exist two category of methods: \begin{inparaenum} \item : . Such relation denotes correlation and causality between the agent in graph structure, regardless of their accessibility in the scenario. (e.g.: player \& hidden gem);
%\item Natural neighboring: the graph edge is formulated as they are adjacently presence in the scenario.(e.g.: link between routers in routing topology)\end{inparaenum}

% Para 2
%In RRL formulation, pair-wise relations were first introduced by \citet{zambaldi2018relational}, using Multi-Head Dot-Product Attention (MHDPA) between interacting entities in the environment for a planning task. 
%A formal GNN feature representation layer in multi-agent RL problems is used by \citet{jiang2020graph}, where a generalized graph convolution function is used to capture the nature of the pre-defined types of relations between interacting agents.% (e.g., greedy, inter-group-competitive, or collaborative).
%Without defining inter-agent relation, \citet{ryu2020multi} pre-cluster the agent in latent space according to prior knowledge, and apply GAT within such cluster. 
%Such method improves the per-game scores and the latter improves the mean reward when relational information being encoded in graph representations. 
%Since \citet{daigavane2021understanding} showed the effectiveness of graph-convolution-based methods in graph with homogeneity feature among node-of-interest and its neighbors, graph-convolution becomes a popular feature representation in this formulation \cite{zambaldi2018relational, jiang2020graph}.  

\author{\IEEEauthorblockN{1\textsuperscript{st} Name Surname}
\IEEEauthorblockA{\textit{Affiliation} \\
email}
\and
\IEEEauthorblockN{2\textsuperscript{nd} Name Surname}
\IEEEauthorblockA{\textit{Affiliation} \\
email}
\and
\IEEEauthorblockN{3\textsuperscript{rd} Name Surname}
\IEEEauthorblockA{Affiliation \\
email}
}

%The majority of these RL approaches mainly employed standard $Q$-learning methods with function approximators such as feed-forward ANNs or linear function approximators \cite{Eckhardt11, Balevi19}. 

%We present our GAQ algorithm
%We propose a RET optimization approach based on Graph Attention $Q$-Network.%Hence, the algorithm includes two components: \textit{(i)} a GAT and \textit{(ii)} a DQN layer.

    %\item \textit{Environment}: $E$, a simulated mobile network in an urban  environment. The environment is depicted in Fig. \ref{fig:environment}, and its parameters are presented in Table \ref{table:sim}. Nodes in the graph represents cells in the networks and edges represents relations between cells.
    
    %In essence, the algorithm uses multi-head graph attention to perform feature augmentation of the target and neighboring nodes. This results in a better state representation, enhancing the pairwise node relations, and resulting in improved performance of the $Q$-learning method. In fact, with such enriched state representation, the agent can better capture neighbors effects such as mutual interference relations between the neighboring nodes.

% Specifically, in step 1 and 2 of the algorithm, each node is parameterized by a weight matrix, with learn-able parameters $W \in \mathbb{R}^{d' \times F}$ (usually $d'>F$). The attention mechanism is parameterized by attention weights $\alpha = (\alpha_{ij})_{(i,j) \in[N]^2}$ and is employed as a convolutional kernel to take feature information from neighboring nodes. The attention weights $\alpha_{ij}$ includes a single-layer feed-forward neural network with non linear activation function (e.g., LeakyReLU with negative input slope), and is parameterized by a weight vector \textbf{a} $\in \mathbb{R}^{2d'}$. In RET optimization, the information of neighboring nodes are less important than the  target node information. Thus, an offset $k>0$ is applied to the self-attention layer in order to give more importance to the target node with respect to the  neighbors features. This offset  ensures both attentions are normalized to be one. In step 3, the attention coefficients are used to compute a higher-level embedding with a linear combination operation, as the aggregating steps in GAT. Multi-head mechanism is applied as well, as we concatenate each attention head's result, to strengthen the robustness of the model. The steps (8-10), updates the loss function in a $Q$-learning fashion.
%\begin{equation}
%    \mathcal{L}(v,w) = [r + \gamma \max_{a\in\mathcal{A}} Q(s_{t+1, i}, a) - Q_w(s_{t,i}, a_{t,i}; v)]^2 
%\end{equation}

%We divide this section in two parts. The first part presents related work in RET optimization methods using RL methods, while the second part presents related work for methods combining GNNs and RL. 



\medskip \noindent \textbf{Graph Neural Networks in Reinforcement Learning}
Various works explored the combination of RL and GNNs methods \cite{jiang2020graph, almasan_deep_2020, zambaldi2018relational, bernardez2021machine, liu2020multi, ryu2020multi}. The majority of these methods, focused on learning expressive feature representations of graph-structured data to represent the state of the agent.

For example, the authors of \cite{jiang2020graph,liu2020multi,bernardez2021machine,ryu2020multi}, introduced GNN as a feature representation layer for building representative state embeddings for multi-agent RL in different applications. Some of the works are framed as Relational Reinforcement Learning (RRL) setting \citet{zambaldi_relational_2018}, in which edges of the graph captures pair wise relation between nodes. 
In our approach, the nodes capturing important relations are the actual physical neighbors in the network graph. 
In addition, we do not use pre-defined relation types (e.g.: collaborative or competitive) between agents as in \cite{jiang2020graph} nor we build homogeneity based on clustering or other inference method within the node adjacencies as \cite{ryu2020multi}. We rather rely on GAT layers to automatically extract the heterogeneity among neighbor relations from the target node reward. Such reward encodes both the agent's and its neighbors' information.

% Para 3
In RL, the main use of GNN is to select neighbor nodes having useful information to the target node state, and encode this information in an efficient manner. To this end, there are two main graph aggregation methods used in the literature. \citet{bernardez2021machine} focused on the path-based aggregation of agent states, where a sequence of agents jointly collaborate towards a common goal. One example of this graph is a routing problen, as data traffic could have long trajectories that associate the router state alongside its path. In a similar application, \citet{almasan_deep_2020} proposed that the state embedding of a router aggregates only the neighboring router's states rather than more distant routers' states. 
The authors proposed a solution to feed all the routers' state embedding to a centralized, single-agent RL solution. 
Multi-agent RL approaches have been compared and shown to outperform these methods~\cite{bernardez2021machine}.
\citet{almasan_deep_2020}'s learnt policy is better performed when generalized to unseen topology structures in the training time.

Our method is also working on the natural graph formulation. By using domain knowledge, we focused on combining adjacent node features from neighboring nodes similar to \citet{almasan_deep_2020}. Yet, we aim to learn multi-agent policies as \citet{bernardez2021machine}. The performance analysis shows that our method is able learn policies in a simple network that can be generalized to more complex topologies.

%as well as the unique impact from each neighboring agent's state. Such state is jointly formulated by messages from second-hop neighbors and neighboring agent's attributes.
%These methods can be considered as if the graph structure is formulated by correlation and causality based on inference, or by naturally formed graph representations. The former methods, originated from Relational Reinforcement Learning (RRL), use GNNs to capture node-wise feature, e.g. neighboring relation and degree. The latter methods, use GNN to perform structural feature extraction which include more topological information. 

%The authors of \cite{jiang2020graph} represent a multi-agent environment as a graph in which the nodes of the graph represent agents and each node has a set of neighbors. The network can generate the $Q$-value as different input levels of latent feature embeddings of the graph. Thereby the network can compute the $Q$ value by knowing the different scope of receptive field information of the graph. 

%\citet{almasan_deep } and \citet{bernardez2021machine} employ a GNN in combination with DQN for optimizing the forwarding strategy of routing networks~\cite{almasan_deep_2020}. %They used a Message Passing Neural Network (MPNN) \cite{gilmer_neural_2017} to update the DQN policy. 
%Our work was originally inspired by this paper and lead to new solutions for antenna optimization using GNNs.

\begin{comment}
To analyze the per-feature contribution to the node's embedding, we suggest an evaluation methodology, called \textit{Dictionary-LOOKUP}, first proposed by \citet{brody2021attentive}.  Specifically, for any two nodes $(i,j) \in\mathcal{E}$ we look at the impact of each of features from node $i$ on node $j$. This is done by "switching off" (setting to $0$) all observation parameter expect the studied one, and "switching on" the studied parameter's observation (setting to be $1$), for node $i$ and $j$ respectively. \\

In \textit{Dictionary-LOOKUP} formulation, according to our observation 
$h_i \in \mathbb{R}^{d}$, we consider a bipartite graph $G_B = (U,V,E)$. We denote $U$ to be the "source node" set and $V$ to be the "neighboring node" set. For $u_m \in U$ denote the $m$-th  observation parameter is "switching on". $v_n \in V$ denote the $n$-th  observation parameter is "switching on". Given $|U| = |V| = d$, for every $u \in U$ and $v \in V$, there exists $(u,v) \in E$. 

By inference on the bipartite graph $G_B$ as we formulated, we visualize the attention strength when different source node feature and neighbour node feature are being "switching on". The attention weight with respect to the observed node attributes on both ends of is illustrated in Fig.\ref{fig:DicLookAttn}.\\
%\begin{figure}[h!]
%    \centering
%    \includegraphics[width = \columnwidth]{figures/DictionaryLookUp.pdf}
%    \caption{\textit{Dictionary-LOOKUP} Graph formulation at size $k = 8$, Each node is assigned with one observed parameter with value $1$, and all rest are $0$. We inference on this graph topology to visualize the attention weight in the trained model. The goal is to analyse per-observed-parameter contribution to the attention.}
%    \label{fig:DicLookGraph}
%\end{figure}
\begin{figure}[h!]
    \centering
    \includegraphics[width = \columnwidth]{figures/DicLookUPAttn.pdf}
    \caption{Attention Visualization in \textit{Dictionary-LOOKUP} Topology, horizontal and vertical axis names denotes observed attributed on the source side and neighboring side of a connected edge, respectively.}
    \label{fig:DicLookAttn}
\end{figure}

\noindent In Fig. \ref{fig:DicLookAttn}, we can observe that the source node features have more impact on edge attention that neighboring node feature, which is aligned with our domain experience in antenna tilt optimization. Also, some observation feature are considered to be related in defining coverage and capacity of a cell. Specifically, $\text{SINR}_{90-\text{SRC}}$ \& $\text{SINR}_{10-\text{DST}}$ and $\text{SINR}_{50-\text{SRC}}$ \&  $\text{SINR}_{50-\text{DST}}$ may be considered as pairs of complementary features, which jointly define the radio coverage in the source node. Indeed, from Fig. \ref{fig:DicLookAttn}, we can observe that such complementary attributes form strong attention, as expected. 
\end{comment}

%In addition, it is usually  these methods to different network topologies.

%In this paper, we propose a Graph Attention $Q$-learning (GAQ) algorithm for tilt optimization. GAQ relies on a graph attention mechanism to select relevant neighbors information, improving the agent state representation, and updates the tilt control policy based on a history of observations using Deep $Q$-Learning (DQN). We show that GAQ efficiently captures important network information and outperforms standard DQN with local information by a large margin. In addition, we demonstrate its ability to generalize to network deployments of different sizes and density.


% Nor we reformulate the system's adjacency as in \cite{zambaldi_relational_2018, ryu2020multi}.

%For example, the authors of   \cite{jiang2020graph,liu2020multi,bernardez2021machine,ryu2020multi}, introduced GNN as a feature representation layer for building representative state embeddings for multi-agent RL in different applications. 
%Some of the works \citet{zambaldi_relational_2018,jiang2020graph} are framed as Relational Reinforcement Learning (RRL) setting, in which edges of the graph captures pair wise relation between nodes. 
% In our approach, the nodes capturing important relations are the actual physical neighbors in the network graph. 
% In addition, we do not use pre-defined relation types (e.g.: collaborative or competitive) between agents as in \cite{jiang2020graph} nor we build nearest neighbor graph based on clustering or other inference method within the node adjacencies as \cite{ryu2020multi}. We rather rely on GAT layers to extract the heterogeneity among neighbors' relation from the target node embedding. %Such reward encodes both the agent's and its neighbors' information.

% Para 3
%In RL, the main use of GNN is to select neighbor nodes having useful information to the target node state, and encode this information in an efficient manner. To this end, there are two main graph aggregation methods used in the literature.
%\citet{bernardez2021machine} focused on the path-based aggregation of agent states, where a sequence of agents jointly collaborate towards a common goal. One example of this graph is a routing problem, as data traffic could have long trajectories that associate the router state alongside its path. In a similar application,
%\citet{almasan_deep_2020} proposed that the state embedding of a router aggregates only the neighboring router's states rather than more distant routers' states. 
%The authors proposed a solution to feed all the routers' state embedding to a centralized, single-agent RL solution. 
%Multi-agent RL approaches have been compared and shown to outperform these methods~\cite{bernardez2021machine}.
%\citet{almasan_deep_2020}'s learnt policy is better performed when generalized to unseen topology structures in the training time.

%Our method is also working on the natural graph formulation. By using domain knowledge, we focused on combining adjacent node features from neighboring nodes similar to \citet{almasan_deep_2020}. Yet, we aim to learn multi-agent policies as \citet{bernardez2021machine}. The performance analysis shows that our method is able learn policies in a simple network that can be generalized to more complex topologies.



%### Long delete text ### 
%as well as the unique impact from each neighboring agent's state. Such state is jointly formulated by messages from second-hop neighbors and neighboring agent's attributes.
%These methods can be considered as if the graph structure is formulated by correlation and causality based on inference, or by naturally formed graph representations. The former methods, originated from Relational Reinforcement Learning (RRL), use GNNs to capture node-wise feature, e.g. neighboring relation and degree. The latter methods, use GNN to perform structural feature extraction which include more topological information. 

%The authors of \cite{jiang2020graph} represent a multi-agent environment as a graph in which the nodes of the graph represent agents and each node has a set of neighbors. The network can generate the $Q$-value as different input levels of latent feature embeddings of the graph. Thereby the network can compute the $Q$ value by knowing the different scope of receptive field information of the graph. 

%\citet{almasan_deep } and \citet{bernardez2021machine} employ a GNN in combination with DQN for optimizing the forwarding strategy of routing networks~\cite{almasan_deep_2020}. %They used a Message Passing Neural Network (MPNN) \cite{gilmer_neural_2017} to update the DQN policy. 
%Our work was originally inspired by this paper and lead to new solutions for antenna optimization using GNNs.


\begin{comment}
\begin{table}
 \caption{Hyper parameter choice.}
 \centering 
 \label{table:hpresult}
 \begin{threeparttable}
    \begin{tabular}{cccc}
    \toprule
    Model & Symbol & Learning rate & Batch size \\
    \midrule\midrule
    DQN  & $\mathbf{\eta_{DQN}}$&  $0.001$ & $100$ \\
    \midrule
    Neighbor DQN & $\mathbf{\eta_{N-DQN}}$& $ 0.001$ & $100$ \\
    \midrule
    GAQ &$\mathbf{\eta_{GAQ}}$& $0.003$ & $64$ \\
    \bottomrule
    \end{tabular}
\end{threeparttable}
\end{table}

\begin{table}[h!]
  \caption{Training hyper-parameters.}
  \label{table:otherhp}
  \centering 
  \begin{threeparttable}
    \begin{tabular}{p{4cm}p{1cm}p{2.5cm}}
    \toprule
    \textbf{Parameter} & \textbf{Symbol} & \textbf{Value} \\
     \midrule\midrule
    Replay buffer size & $T_b$& $1500$  \\
    \midrule
    Initial exploration rate &$\varepsilon_\text{init}$ &  $1$ \\
    \midrule
    Final exploration rate & $\varepsilon_\text{final}$&  $0.01$\\
    \midrule
    Number of neurons  & $N_{h}$ &  $[100,50,20]$\\
    \midrule
    Activation function & $\sigma$ &  ReLU \\
    \midrule
    Number of attention heads & $K_\text{attn}$ &  $6$ \\
    \midrule
    Episode length & $T_\text{episode}$ &  $20$ \\
    \midrule
    Batch size & $T_\text{batch}$ & $64$ \\
    \midrule
    Number of epochs & $N_\text{epoch}$ & $20$ \\
    \bottomrule
    \end{tabular}
\end{threeparttable}
\label{tab:train_hyp}
\end{table}
\end{comment}
